SoLo T-DIRL: Socially-Aware Dynamic Local Planner based on Trajectory-Ranked Deep Inverse Reinforcement Learning

This work proposes a new framework for a socially-aware dynamic local planner in crowded environments by building on the recently proposed Trajectory-ranked Maximum Entropy Deep Inverse Reinforcement Learning (T-MEDIRL). To address the social navigation problem, our multi-modal learning planner explicitly considers social interaction factors, as well as social-awareness factors into T-MEDIRL pipeline to learn a reward function from human demonstrations. Moreover, we propose a novel trajectory ranking score using the sudden velocity change of pedestrians around the robot to address the sub-optimality in human demonstrations. Our evaluation shows that this method can successfully make a robot navigate in a crowded social environment and outperforms the state-of-art social navigation methods in terms of the success rate, navigation time, and invasion rate.

==> discussion.tex <==
\section{Discussions and Limitations}
\label{sec:discussion}
\tk{If possible talk about quality of path, compare the run time Vs estimated time of tour, move\_base failures}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width = \textwidth/2]{figures/umma.jpg}
%     \caption{Caption}
%     \label{fig:umma_cube}
% \end{figure}
% The study has focused on designing a behavior planning pipeline for a socially assistive robot. The recommendation for a global (tour) planning mechanism is based on a travelling salesman problem that optimizes tours for optimal visitor learning experience. The initial guess of the study has been to show how to encode constraints on human attention capacity, however the demands for each node in the graph were manually assigned for now. The efficacy of the experiment can benefit from future Human-in-the-loop testing for optimal learning experience. Further, we would like to bring in domain knowledge from experienced museum educationist (our collaborators at University of Michigan Museum of Arts(UMMA)), to help us craft user models that could help design better tours for an art education experience at a museum. 

% The learning based agent relies on very little information from the environment to make navigation decisions, making it an ideal agent to adapt to changes in the environment that inherently happen over time. Artworks move, furniture is re-arranged, changing the space and the map. With the proposed agent, we assume that environment is actually unknown, so these changes can be handled. However, in making the same assumption, we may sometimes end up taking longer paths to reach a goal when we could have trusted the map more, and found a shorter path. This balance on how much of the information from the environment is reliable and should be used is an open ended question for the problem. Our next approach in this direction would be to use a hybrid model where, a part of a plan uses a shortest path planner, while a re-planning component is a learning based agent. Finally, the current study has not evaluated language based navigation agents, which is necessary when moving towards multi-modal feedback for behavior planning in SARs.

==> experiments.tex <==
\section{Experimental Setup}
\label{sec:implementation}

The last part of the problem is to set up the pipeline that would let the two layers of planning work together. We have chosen to implement this is ROS for two reasons. One, ROS communication protocol is easy to use, reliable and widely popular in the robotics community. Second, our final product will be running this architecture to give tours using a Fetch robot, which also runs on ROS. Thus, shifting everything from simulation to real world experiments is easier, with minimal change to code. 

For this study, we have focused on giving a house tour in Matterport3D dataset, simulated in the Habitat simulation environment. We build a ROS interface that could then communicate with the Habitat-lab and the backend Habitat-sim package. The experiments were done using Ros-Noetic on an ubuntu 20.04 LTS system. We used Noetic to stay compatible with Python 3.6 version, that is used for Habitat environment. To easily resolve package dependencies for new install, both ROS and Habitat package were built in a conda environment \citep{robotstack}.

The ROS wrapper over Habitat-sim, was used to extract image (RGB and depth) data and published as ROS messages visualized in Rviz at a sensor rate of 50 Hz. The top-down map was read as an occupancy grid map and the transforms were published between the map and world coordinates. Finally the tour planning node was used to publish a plan, subscribed to by the local planner node, which would then create a new episode in the Habitat-environment and extract the agent policy and execute those actions in simulation. 

